From Reading to Compressing: Exploring the Multi-document Reader for Prompt Compression

Large language models (LLMs) have achieved significant performance gains using advanced prompting techniques over various tasks. However, the increasing length of prompts leads to high computational costs and often obscures crucial information. Prompt compression has been proposed to alleviate these issues, but it faces challenges in (i) capturing the global context and (ii) training the compressor effectively. To tackle these challenges, we introduce a novel prompt compression method, namely Reading To Compressing (R2C), utilizing the Fusion-in-Decoder (FiD) architecture to identify the important information in the prompt. Specifically, the cross-attention scores of the FiD are used to discern essential chunks and sentences from the prompt. R2C effectively captures the global context without compromising semantic consistency while detouring the necessity of pseudo-labels for training the compressor. Empirical results show that R2C retains key contexts, enhancing the LLM performance by 6% in out-of-domain evaluations while reducing the prompt length by 80%.

==> Figures_tex/case_study_multidoc_tok.tex <==
\begin{figure*}[htb]
\centering
\begin{tcolorbox}[colframe=black,colback=white!10!white,title=Case study of MultiDocQA task in LongBench,fonttitle=\bfseries]

\textbf{R2C Compressed Prompt with $T=1,000$ (1,028 tokens, Original length: 7,614 tokens)}\\
Answer the question based on the given passages. Only give me the answer and do not output any other words.
\newline The following are given passages.
 
\colorbox{instructionbg}{\parbox{\dimexpr\linewidth-2\fboxsep}{Funeral services are held for Carolyn, and she is buried in the Collins family mausoleum.
\newline Cast
\newline Production
\newline Dark Shadows producer Dan Curtis began pitching the idea of a film based on his gothic soap opera sometime in 1968.

~~~~~~~~~$\vdots$


The story was very loosely based on the "parallel-time" sequence of the TV series and centered on the show's other popular male lead, Quentin Collins, played by David Selby. \hl{Night of Dark Shadows was shot in six weeks on a budget of \$900,000 and released in 1971}, after the show had left the air. It was not unsuccessful but was less successful than its predecessor.

Hall's script, developed in conjunction with Curtis, was a wistful tale of gothic romance and supernatural reincarnation, bolstered by credible performances from David Selby, Kate Jackson, and Grayson Hall. When filming completed without major problems, Curtis set about editing the final film, which proved far denser and more complex than House of Dark Shadows.

Home media

Night of Dark Shadows and House of Dark Shadows were released on VHS on September 1, 1998, and on DVD and Blu-ray on October 30, 2012 by Warner Home Video.
See also

~~~~~~~~~$\vdots$

Lizzie Hopley – Street Walker
\newline Richard Halpern – Announcer
\newline Eric Wallace – Conductor
\newline External links
\newline Dark Shadows - 2.0 Kingdom Of The Dead Box Set
\newline Passage 8:
\newline Alkohol
\newline \hl{Alkohol (English: Alcohol) is a 1919 German silent drama film} directed by Ewald André Dupont and Alfred Lind and starring Wilhelm Diegelmann, Ernst Rückert, and Georg H. Schnell. It was his first major melodrama, and represented a breakthrough in his career.
\newline Passage 9:
\newline Nightstand (disambiguation)
\newline A nightstand is a small bedside table.}}


Now, answer the following question based on the above text, only give me the answer and do not output any other words.

\colorbox{questionbg}{\parbox{\dimexpr\linewidth-2\fboxsep}{Question: Which film came out earlier, Alkohol or Night Of Dark Shadows?

Answer:}}

\vspace{0.5cm}

\textbf{Prediction (GPT-3.5-turbo-1106)}
\newline Alkohol

\vspace{0.5cm}

\textbf{Ground truth}
\newline Alkohol

\end{tcolorbox}
\caption{Case study on the 2WikiMultihopQA dataset (MultiDoc) in the LongBench benchmark. The \hl{purple colorbox} indicates the core information to generate answers.}\label{fig:case_multidoc}
\end{figure*}


==> Tables/tab_dataset.tex <==
\begin{table}[t]\small
\begin{footnotesize}
\begin{tabular}{c|ccc|c|c}
\toprule
Dataset & train & dev & test & R@20 & \# pos/q \\ \midrule
NQ      & 79,168            & 8,757           & 3,610            & 0.87               & 4.5                      \\
TQA     & 78,785            & 8,837           & 11,313           & 0.86               & 8.9                      \\ \bottomrule
\end{tabular}
\end{footnotesize}
\caption{Data statistics. \# pos/q indicates the average number of passages that have the answer span per the question. R@$K$ is one if there exists a positive among the $K$ passages and zero. R@20 and \# pos/q are for the training dataset using the retriever~\cite{emnlp/KarpukhinOMLWEC20/DPR} trained by~\citet{iclr/IzacardG21/FiD-KD}.}
\label{tab:dataset}
\end{table}

==> Tables/tab_dataset_stat_nq.tex <==
\begin{table}\footnotesize
\setlength{\tabcolsep}{1.9pt} 
\renewcommand{\arraystretch}{1}
\centering
% \usepackage{multirow}
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Source} & \multirow{2}{*}{Avg len} & \multirow{2}{*}{Metric} & \multicolumn{3}{c}{\# data} \\
 &  &  & Train & Dev (subset) & Test \\ \midrule
Wikipedia & 3,018 & Span EM & 79,168 & 1,757 & 3,610 \\ \bottomrule
\end{tabular}

\caption{Detailed statistics of Natural Questions~\cite{tacl/KwiatkowskiPRCP19/NQ}. `Source' denotes the original source of the context. `Avg len' is the average length of test set computed by the GPT-3.5 tokenizer.}
\label{tab:statistic_nq}


\end{table}

==> Tables/tab_labelcomparison.tex <==
\begin{table}[t]\small
\centering
\begin{tabular}{c|cc|cc}
\toprule
\begin{tabular}[c]{@{}c@{}}Evidence\\ label\end{tabular} & \begin{tabular}[c]{@{}c@{}}NQ dev\\ (EM)\end{tabular}    & \# pos. & \begin{tabular}[c]{@{}c@{}}TQA dev\\ (EM)\end{tabular} & \# pos. \\ \midrule
-                                                        & 47.8 \scriptsize $\pm$ 0.16 & -       & 67.4 \scriptsize $\pm$ 0.12 & -       \\ \midrule
Ans. span                                              & 48.5 \scriptsize $\pm$ 0.21 & 4.5     & 67.7 \scriptsize $\pm$ 0.16     & 8.9     \\
ChatGPT                                                  & \textbf{48.9} \scriptsize $\pm$ 0.13 & 4.0     & 67.7 \scriptsize $\pm$ 0.20      & 8.3 \\
MythoMax                                                 & 48.8 \scriptsize $\pm$ 0.23 & 2.8     & \textbf{67.8} \scriptsize $\pm$ 0.18   & 6.5     \\ \bottomrule
\end{tabular}
\caption{Model performance with different evidence labels. \# pos. denotes the average number of positive labels in top-20 passages.}
\label{tab:label_comparison}
% \vspace{-3mm}
\vskip -0.1in
\end{table}

==> Tables/tab_nq_oracle.tex <==
\begin{table}[t]\small
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{c|}{\textbf{Compression}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}NQ-oracle\\ (Span EM)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ \# toks\end{tabular}} & \textbf{/org.} \\ \toprule
\multicolumn{1}{c|}{-}                    & \multicolumn{1}{c|}{87.8}                                                                   & 156                                                             & 100.0\%        \\ \midrule
\multicolumn{4}{c}{1.5x compression (target tokens: 120)}                                                                                                                                                               \\ \midrule
\multicolumn{1}{c|}{LLMLingua-2}          & \multicolumn{1}{c|}{}                                                                       &                                                                 & 0.0\%          \\
\multicolumn{1}{c|}{LongLLMLingua}        & \multicolumn{1}{c|}{}                                                                       &                                                                 & 0.0\%          \\ \midrule
\multicolumn{1}{c|}{R2C-sentence}         & \multicolumn{1}{c|}{\textbf{86.1}}                                                          & 116                                                             & 74.2\%         \\ \midrule
\multicolumn{4}{c}{2x compression (target tokens: 80)}                                                                                                                                                               \\ \midrule
\multicolumn{1}{c|}{LLMLingua-2}          & \multicolumn{1}{c|}{}                                                                       &                                                                 & 0.0\%          \\
\multicolumn{1}{c|}{LongLLMLingua}        & \multicolumn{1}{c|}{}                                                                       &                                                                 & 0.0\%          \\ \midrule
\multicolumn{1}{c|}{R2C-sentence}         & \multicolumn{1}{c|}{\textbf{77.3}}                                                          & 79                                                              & 50.6\%         \\ \bottomrule
\end{tabular}
\label{tab:nq_oracle}
\end{table}
